Thick points of 4D critical branching Brownian motion

We study the thick points of branching Brownian motion and branching random walk with a critical branching mechanism, focusing on the critical dimension $d = 4$. We determine the exponent governing the probability to hit a small ball with an exceptionally high number of pioneers, showing that this has a second-order transition between an exponential phase and a stretched-exponential phase at an explicit value ($a = 2$) of the thickness parameter $a$. We apply the outputs of this analysis to prove that the associated set of thick points $\mathcal{T}(a)$ has dimension $(4-a)_+$, so that there is a change in behaviour at $a=4$ but not at $a = 2$ in this case. Along the way, we obtain related results for the nonpositive solutions of a boundary value problem associated to the semilinear PDE $\Delta v = v^2$ and develop a strong coupling between tree-indexed random walk and tree-indexed Brownian motion that allows us to deduce analogues of some of our results in the discrete case. We also obtain in each dimension $d\geq 1$ an infinite-order asymptotic expansion for the probability that critical branching Brownian motion hits a distant unit ball, finding that this expansion is convergent when $d\neq 4$ and divergent when $d=4$. This reveals a novel, dimension-dependent critical exponent governing the higher-order terms of the expansion, which we compute in every dimension.

==> sections_tex_files/elementary_g.tex <==
\red{This section is useless now since everything is contained in Lemma \ref{L:v_ODE}}

\begin{lemma}\label{L:elementary_g}
For $\lambda >0$, let $g_\lambda$ be the unique maximal solution to
\[
\left\{ \begin{array}{l}
g'' + 2g' = g^2, \\
g(0) = 0, \quad 
g'(0) = -\lambda.
\end{array} \right.
\]
$g_\lambda$ is defined on $(0,\infty)$, i.e. does not explode in finite time. Moreover, for any $0< \lambda_1 < \lambda_2$, we have
\[
g_{\lambda_1}(x) > g_{\lambda_2}(x)
, \quad \quad x >0.
\]
\end{lemma}


\begin{proof}
Let $L>0$ be large. We are going to prove that solutions are defined on $[0,L]$ and that they do not overlap on that interval.

Denote by $R = e^L$. For any $s<0$, define as before
\[
\mathsf{g}_{s}(x) := r^2 \EXPECT{r,R}{ 1 - (1-s)^N}, \quad \quad \text{where}~ r = R/e^x.
\]
For all $s < 0$, we denote by $\lambda(s) = -\mathsf{g}_s'(0) \in (0,\infty)$.
Since $\mathsf{g}_s$ satisfies $\mathsf{g}_s'' + 2\mathsf{g}_s' = \mathsf{g}_s^2$, for all $s<0$, $\mathsf{g}_s = g_{\lambda(s)}$.

The lemma will follow from the fact that the map $\lambda : s \in (-\infty,0) \mapsto \lambda(s) \in (0,\infty)$ is a decreasing bijection. Indeed, assuming this fact, for all $0<\lambda_1<\lambda_2$, there exist $s_2 < s_1 < 0$ such that $g_{\lambda_i} = \mathsf{g}_{s_i}$, $i=1,2$. Then it is clear from the probabilistic definition of $\mathsf{g}_{s_i}$ that the solutions are well defined on $[0,L]$ and that $\mathsf{g}_{s_1} > \mathsf{g}_{s_2}$ on $[0,L]$.

We now prove that $\lambda : s \in (-\infty,0) \mapsto \lambda(s) \in (0,\infty)$ is indeed a decreasing bijection. The fact that $\lambda$ is decreasing is clear: as already noticed, if $s_2 < s_1 < 0$, then $\mathsf{g}_{s_1} > \mathsf{g}_{s_2}$ on $[0,L]$ implying that $- \lambda(s_1) \geq -\lambda(s_2)$. Furthermore, $\lambda(s_1)$ cannot agree with $\lambda(s_2)$ by uniqueness of solutions with fixed initial value and derivative.


$\lambda(0) = 0$ and integrating the relation $\gs_s'' + 2\gs'_s \geq 0$ from $0$ to $L$ gives
\[
s = \gs_s(L) \geq \frac12 \gs_s'(0) \left( 1 - e^{-2L} \right) = -\frac12 \lambda(s) \left( 1 - e^{-2L} \right)
\]
which shows that $\lambda(s) \to \infty$ as $s \to - \infty$. To conclude, we only need to show that $\lambda$ is a continuous function of $s$.

\red{It remains to prove that $\lambda$ is continuous on $(-\infty,0]$
 Excursion...}
\end{proof}


\begin{comment}
\begin{proof}
\red{AJ: I still have to work on the proof}

Let $0< \lambda_1 < \lambda_2$ and define $f = g_{\lambda_1} - g_{\lambda_2}$. Our goal is to prove that $f$ remains positive. We have $f(0)=0$ and $f'(0) >0$. Let $u = \inf \{ x: f'(x) = 0 \}$. Clearly, for all $x \in (0,u]$, $f(x) >0$, so we will focus on the interval $[u,\infty)$. Let $x_\infty := \inf\{ x>u: f(x) = 0 \}$. Our goal is to show that $x_\infty = +\infty$, but let us first prove that for all $x \in [u,x_\infty)$, $f'(x) \leq 0$, that is, $f$ is nonincreasing on $[u,x_\infty)$.
Using the ODE satisfied by $g_{\lambda_1}$ and $g_{\lambda_2}$, we see that $f$ satisfies
\begin{equation}
\label{E:proof_L_g1}
f'' + 2f' = f (g_{\lambda_1} + g_{\lambda_2}).
\end{equation}
In particular, on $[u,x_\infty)$, $f'' + 2f' \leq 0$. Integrating this inequality shows the desired claim: for all $x \in [u,x_\infty)$,
\[
f'(x) = e^{-2x} \int_u^x (f'' + 2f') \leq 0.
\]

We will now show that $x_\infty = +\infty$. We proceed by contradiction and we assume that $x_\infty < \infty$.
Let $p_0 \geq 1$ be large enough so that $f(u) > 2^{-p_0}$ and define for all $ p \geq p_0$,
\[
x_p := \inf \{ x > u: f(x) \leq 2^{-p} \}.
\]
By continuity, $x_p \to x_\infty$. We are going to use \eqref{E:proof_L_g1} and we argue that we have a good control of the right hand side of \eqref{E:proof_L_g1} when $x \in [x_p,x_{p+1}]$. Indeed, by *** there exists $c,C>0$ such that for all $x \geq u$,
\[
-\frac{C}{x} \leq g_{\lambda_1}(x) + g_{\lambda_2}(x) \leq -\frac{c}{x}.
\]
Also, by definition of $x_p$ and because $f$ is nonincreasing on $[x_p,x_{p+1}]$, for all $x \in [x_p, x_{p+1}]$, $2^{-p-1} \leq f(x) \leq 2^{-p}$. Therefore, on that interval, we have
\[
-C 2^{-p} \frac{1}{x} \leq f''(x) + 2f'(x) \leq -c 2^{-p-1} \frac{1}{x}.
\]
After integration, it gives
\[
-C 2^{-p} \int_{x_p}^{x_{p+1}} \frac{1}{x} e^{2x} \d x \leq f'(x_{p+1})e^{2x_{p+1}} - f'(x_p) e^{2x_p} \leq -c 2^{-p-1} \int_{x_p}^{x_{p+1}} \frac{1}{x} e^{2x} \d x
\]
\end{proof}
\end{comment}



==> sections_tex_files/gsmall4.tex <==
This section proves Lemma \ref{L:g_small_lambda}.




\begin{proof}
\begin{figure}
\centering
\includegraphics[width=0.3\textwidth]{images/g.jpeg}
\includegraphics[width=0.3\textwidth]{images/"gg'_drawing.jpeg"}
\caption{Left: Plot of the function $g$ in blue. The orange line corresponds to $-C_0/(2L)$.
Right: Schematic representation of the phase portrait of $g$.}
\end{figure}

\begin{figure}
\includegraphics[width=0.2\textwidth]{images/g1.jpeg}
\includegraphics[width=0.4\textwidth]{images/g2.jpeg}
\caption{Left: $g'$ against $g$ drawn for $x \in [0,x_0]$.
Right: $L g'$ against $g$ drawn for $x \in [x_0,L]$. Note the scaling.}
\end{figure}

Let $\mu >0$, $\lambda = \mu/x$ and let us simply write $g$ instead of $g_{\lambda}$ in this proof. We will keep track of the dependence in $\mu$ in the constants and $O(1)$ in this proof. Therefore, all the constants and $O(1)$ in this proof will be independent of $\mu$.
Let 
\[
x_0 := \inf \{ y > 0: g'(y) = 0 \}
\quad \text{and} \quad
x_1 := \inf \{ y>x_0: g(y)^2 - 2g'(y) = 0 \}.
\]
We will show that
\begin{equation}\label{E:proof_ODE1}
x_0 = \frac{1}{2} \log \frac{8}{\lambda} + O \left( \lambda \log \frac{1}{\lambda} \right)
\quad \text{and} \quad
g(x_0) = -\left((1+ O \left( \lambda \right) \right) \frac{\lambda}{2},
\end{equation}
\begin{equation}\label{E:proof_ODE2}
x_1 - x_0 \leq \frac12 + O(\lambda)
\quad \text{and} \quad
|g(x_1) - g(x_0)| \leq \frac{\lambda^2}{16} (1+O(\lambda))
\end{equation}
and for all $y \geq x_1$,
\begin{equation}\label{E:proof_ODE3}
0 \leq 2g'(y) - g(y)^2 \leq (1+O(\lambda)) \frac{\lambda^3}{16}.
\end{equation}
Let us assume these estimates for now and let us explain how we conclude from this.


Let $\nu = 1 / (\mu+4)>0$ be a parameter and let $x_2 := \inf \{ y>x_1: g(y) \leq - \nu \lambda \}$. On $[x_1,x_2]$, $|g|$ is larger than $\nu \lambda$, so \eqref{E:proof_ODE3} implies that
\[
\frac12 g^2 \leq g' \leq (1+O(\lambda))\left( \frac12 + \frac{\lambda}{16 \nu^2} \right) g^2 \quad \text{on~} [x_1,x_2].
\]
Integrating this relation between $x_1$ and $x_2$ yields
\begin{equation}
\label{E:proof_ODE11}
\frac12 (x_2 - x_1) \leq \frac{1}{g(x_1)} - \frac{1}{g(x_2)} \leq (1+O((\mu^2+1)\lambda)) \frac12 (x_2 - x_1).
\end{equation}
By \eqref{E:proof_ODE1} and \eqref{E:proof_ODE2}, $x_1 = o(1/\lambda)$ and $g(x_1) = - \lambda/2 (1+O(\lambda))$ and by definition of $x_2$, $g(x_2) = -\nu \lambda$. This implies that
\[
x_2 = (1+O((\mu^2+1)\lambda)	) \left( \frac{2}{\nu} - 4 \right) \frac{1}{\lambda}
\geq (1+O((\mu^2+1)\lambda)	) 2x
\]
thanks to this choice of $\nu$. In particular, if $\lambda$ is small enough, $x_2 > x$ and we can apply \eqref{E:proof_ODE11} to $x$ instead of $x_2$ to find that
\[
g(x) = - \left( 1 + \frac{O(\log(\mu/x) + O((\mu^2+1)\mu)}{x} \right) \frac{2\mu}{\mu + 4} \frac{1}{x}.
\]
This shows the desired statement. It now remains to prove \eqref{E:proof_ODE1}, \eqref{E:proof_ODE2} and \eqref{E:proof_ODE3}.



$\bullet~$ \emph{Proof of \eqref{E:proof_ODE1}:}
Using the ODE satisfied by $g$ can be rewritten as
\begin{equation}
\label{E:proof_ODE10}
(g' e^{2y})' = g(y)^2 e^{2y}, \quad y \geq 0.
\end{equation}
In particular the left hand side is non negative. Integrating between 0 and $y$ leads to
\begin{equation}
\label{E:proof_ODE9}
g(y) \geq - \frac{\lambda}{2} (1-e^{-2y}).
\end{equation}
This lower bound on $g$ gives an upper bound on $g^2$. Plugging this upper bound back to \eqref{E:proof_ODE10} gives
\[
g'(y) e^{2y} + \lambda \leq \int_0^y \left( \frac{\lambda}{2} \right)^2 (e^z-e^{-z})^2 \d z
= \frac14 \lambda^2 ( \sinh(2y) - 2y ).
\]
Rearranging the above inequality, we have
\begin{equation}
\label{E:proof_ODE6}
g'(y) \leq - \lambda e^{-2y} + \frac{1}{8} \lambda^2 \left( 1 - e^{-4y} - 4ye^{-2y} \right).
\end{equation}
In particular, we see that if $C>0$ is large enough, for all $y \leq \frac{1}{2} \log \frac{8}{\lambda} - C \lambda$, $g'(y)$ stays negative. In other words,
\begin{equation}
\label{E:proof_ODE7}
x_0 \geq \frac{1}{2} \log \frac{8}{\lambda} - C \lambda.
\end{equation}
We will now provide an upper bound on $x_0$. Integrating \eqref{E:proof_ODE6} gives
\begin{align*}
g(y) & \leq - \frac{\lambda}{2} \left( 1 - e^{-2y} \right) + \frac{1}{8} \lambda^2 \left( y - \frac{1-e^{-4y}}{4} + 2y e^{-2y} - (1-e^{-2y}) \right) \\
& \leq - \left( \frac{\lambda}{2} - C \lambda^2 (1+y) \right) \left( 1 - e^{-2y} \right).
\end{align*}
In particular, we see that for all $y \in [0,\log (1/\lambda)]$,
\begin{equation}
\label{E:proof_ODE8}
g(y) \leq - \frac{\lambda}{2} \left(1 - C \lambda \log \frac{1}{\lambda} \right) \left( 1 - e^{-2y} \right).
\end{equation}
Recall that we obtained the upper bound \eqref{E:proof_ODE6} on $g'$ from the lower bound \eqref{E:proof_ODE9} on $g$. Similarly, the upper bound we now have on $g$ leads to the following lower bound on $g'$: for all $y \in [0,\log (1/\lambda)]$,
\[
g'(y) \geq - \lambda \left(1 - C \lambda \log \frac{1}{\lambda} \right) e^{-2y} + \frac{1}{8} \lambda^2 \left(1 - C \lambda \log \frac{1}{\lambda} \right)^2 \left( 1 - e^{-4y} - 4ye^{-2y} \right).
\]
This shows that $g'$ has to vanish at some point $y$ smaller that $\frac{1}{2} \log \frac{8}{\lambda} + C \lambda \log \frac{1}{\lambda}$ for some constant $C>0$ large enough. This is the desired upper bound on $x_0$. Together with \eqref{E:proof_ODE7}, this shows the estimate \eqref{E:proof_ODE1} on $x_0$. The estimate on the value of $g(x_0)$ follows from \eqref{E:proof_ODE9} and \eqref{E:proof_ODE8}.




$\bullet~$ \emph{Proof of \eqref{E:proof_ODE2}:}
Let $\tilde{x}_1 := \inf \{y \geq x_0: g'(y) \geq \frac{\lambda^2}{8} \}$. We have $x_1 \leq \tilde{x}_1$. 
On $[x_0,\tilde{x}_1]$, $|g'| \leq \frac{\lambda^2}{8}$ which gives 
\begin{equation}\label{E:proof_ODE4}
|g(\tilde{x}_1) - g(x_0)| \leq \frac{\lambda^2}{8} (\tilde{x}_1 - x_0).
\end{equation}
Now, because $g \leq 0$, we have $g'' \geq g^2$. $|g|$ is decreasing on $[x_0,\tilde{x}_1]$, so on this interval we have
\[
g'' \geq g(\tilde{x}_1)^2 \geq \left( g(x_0) - \frac{\lambda^2}{8} (\tilde{x}_1 - x_0) \right)^2_+.
\]
Integrating this inequality between $x_0$ and $\tilde{x}_1$ gives
\[
\frac{\lambda^2}{8} = g'(\tilde{x}_1) - g'(x_0) \geq  \left( g(x_0) - \frac{\lambda^2}{8} (\tilde{x}_1 - x_0) \right)^2_+ (\tilde{x}_1 - x_0)
\]
which yields $\tilde{x}_1 - x_0 \leq \frac{1}{2} + O(\lambda)$. We have obtained that $x_1 - x_0 \leq \tilde{x}_1 - x_0 \leq \frac{1}{2} + O(\lambda)$. Going back to \eqref{E:proof_ODE4} (with $x_1$ instead of $\tilde{x}_1$), we have also obtained that
\[
|g(x_1) - g(x_0)| \leq \frac{\lambda^2}{16} (1+O(\lambda)).
\]
This proves \eqref{E:proof_ODE2}.

$\bullet~$ \emph{Proof of \eqref{E:proof_ODE3}:}
Let $\delta(y) := 2g'(y) - g(y)^2$. We have $\delta'(y) = -2 \delta(y) - 2 g(y) g'(y)$. Hence at the point where the maximum of $\delta$ is reached, $\delta'$ vanishes showing that $\max_{y \geq x_1} \delta(y) \leq \max_{y \geq x_1} |g g'(y)|$. Since $g$ and $g'$ are both non increasing on $[x_1,\infty)$, $\max_{y \geq x_1} \delta(y) \leq |gg'(x_1)|$.
\end{proof}


==> sections_tex_files/od_stuff_outer.tex <==

\begin{lemma}\label{L:unique_family}
There exists a unique family of functions $f_{s} : [0,\infty) \to [0,1]$, $s \in [0,1]$ satisfying the following properties:
\begin{itemize}
\item
For all $x \geq 0$, $s \in [0,1] \mapsto f_{s}(x)$ is analytic;
\item
For all $n \geq 2$, $\frac{\partial^n f_{s}(x)}{\partial s^n}\vert_{s = 0} \to 0$ as $x \to \infty$;
\item
For all $s \in [0,1]$, $f_{s}(0) = s$, $f_s$ is twice differentiable and $f_{s}'' + 2f_{s}' = f_{s}^2$ on $(0,\infty)$.
\end{itemize}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{L:unique_family}]
We focus on the uniqueness part of this statement. The existence will follow from the fact that for any fixed $R \geq 1$, the functions $g_{s,R}$ satisfy the assumptions. See the proof of Lemma \ref{L:invariance}.
Let $f_{s}, s \in [0,1]$ be such functions. By the analyticity hypothesis, we can write 
\[
f_{s}(x) = e^{-2x} s \sum_{n=0}^\infty \alpha_n(x) s^n,
\quad \quad x \geq 0, \quad s \in [0,1].
\]
Because $f_{s}(0) = s$ for all $s \in [0,1]$, we have $\alpha_0(x) = 1$ for all $x \geq 0$.
The ODE satisfied by $f_{s}$ translates to the following equations for the functions $\alpha_n$:
\begin{equation}
\label{E:alpha_ODE}
\forall n \geq 0, \quad -2\alpha_{n+1}' + \alpha_{n+1}'' = e^{-2x} \sum_{k=0}^n \alpha_k \alpha_{n-k}.
\end{equation}
The initial value $f_{s}(0) = s$ fixes the initial values $\alpha_n(0) = 0$ for all $n \geq 1$. The hypothesis on the partial derivative of $f_{s}(x)$ with respect to $s$ implies that for all $n \geq 1$, $e^{-2x} \alpha_n(x) \to 0$ as $x \to \infty$. We now show by induction that for all $n \geq 0$, $\alpha_n$ is uniquely determined and $\alpha_n(x)$ converges to some finite value as $x \to \infty$. The initial case $n=0$ is clear. Let $n \geq 0$ and assume that this is true for all $k \leq n$. Let $A = \sum_{k=0}^n \alpha_k \alpha_{n-k}$. Integrating the equation \eqref{E:alpha_ODE} leads to
\[
\alpha_{n+1}'(x) e^{-2x} - \alpha_{n+1}'(0) = \int_0^x A(y) e^{-4y} \d y.
\]
By the induction hypothesis, $A$ stays bounded at infinity, so the integral $\int_0^\infty A(y) e^{-4y} \d y$ converges. $\alpha_{n+1}$ can stay negligible compared to $e^{2x}$ as $x \to \infty$, only if $\alpha_{n+1}'(0) = - \int_0^\infty A(y) e^{-4y} \d y$. We deduce that
\[
\alpha_{n+1}(x) = - \int_0^x e^{2z} \left( \int_z^\infty A(y) e^{-4y} \d y \right) \d z.
\]
Since $A(x)$ converges as $x \to \infty$, $\alpha_{n+1}$ also converges to some finite value. It concludes the induction proof.
These coefficients can be explicitely computed using this approach. For instance,
\begin{align*}
\alpha_1(x) & = - \frac{1}{8} (1-e^{-2x}),
\quad \quad \alpha_2(x) = \frac{1}{96} (1-e^{-2x}) (2-e^{-2x}), \\
\alpha_3(x) & = - \frac{1}{9216} (1-e^{-2x}) (37 - 29e^{-2x} + 7 e^{-4x} ).
\end{align*}
Overall, we have shown that $f_{s}$ is uniquely determined concluding the proof of the lemma.
\end{proof}




\begin{proof}[Proof of Lemma \ref{L:invariance}]
$f_{t_0,R}$ satisfies
\[
\left\{
\begin{array}{l}
f_{t_0,R}'' + 2f_{t_0,R}' = f_{t_0,R}^2 \quad \text{in} \quad (0,\infty), \\
f_{t_0,R}(0) = t_0.
\end{array}
\right.
\]
For all $x \geq 0$, $t_0 \in [0,1] \mapsto f_{t_0,R}(x)$ is analytic. We should be able to show that for all $n \geq 1$, $R \geq 1$,
\[
\limsup_{x \to \infty} R^2 \EXPECT{e^{-x}R}{ \left( \frac{N_R}{R^2} \right)^n } < \infty.
\]
We do not need any uniformity in $R$ here! So actually, what we really need to show is that for all $n \geq 1$, $R \geq 1$,
\[
\limsup_{x \to \infty} \EXPECT{e^{-x}R}{ \left( N_R \right)^n } < \infty.
\]
This would imply that for all $R \geq 1$, $n \geq 1$,
$\frac{\partial^n f_{t_0,R}(x)}{\partial t_0^n}\vert_{t_0 = 0} = O(e^{-2x}) \to 0$ as $x \to \infty$. We can then conclude using Lemma \ref{L:unique_family}.
\end{proof}


\subsection{Convergence of the number of pioneers on the outer sphere}




\begin{proof}[\red{Old sketch of proof below}]
We might have to specify some behaviour at infinity to ensure that, as a function of the starting point in the sphere, the Laplace transform stays smooth at the origin. For instance, requiring that
\[
e^{2x} (f_{t_0}'(x) + 2f_{t_0}(x)) \to 0 \quad \quad \text{as} \quad x \to \infty,
\]
is the same as requiring that the derivative of the Laplace transform at the centre of the sphere vanishes (which holds by symmetry):
\[
\frac{\d}{\d y} \EXPECT{y}{\left( 1 - \frac{t_0}{R^2} \right)^{N_R} } \Big\vert_{y=0} = 0.
\]

\red{Let's be more precise.}
It seems that the functional equation $f_{f_{t_0}(y)}(x) = f_{t_0}(x+y)$ fixes this extra degree of freedom! This equation requires for all $x,y >0$,
\begin{align*}
\alpha_1(x+y) & = \alpha_1(y) + e^{-2y} \alpha_1(x) \\
\alpha_2(x+y) & = \alpha_2(y) + e^{-4y} \alpha_1(x) + 2 e^{-2y} \alpha_1(x) \alpha_1(y) \\
& \vdots
\end{align*}
It is a bit strange since I would have expected to recover the same equations. For instance, differentiating the first equation above w.r.t. $x$ and then w.r.t. $y$ implies that
\[
\alpha_1'' + 2 \alpha_1' = 0
\]
which is different than the ODE \eqref{E:alpha_ODE}. Together, these equations determine a unique solution for $\alpha_1$! \red{Continue here! Make sure that I really get two different sets of equations}




\end{proof}




\subsection{Identifying the limit}


Assume that for all $x>0$, \[
\frac{N_R}{R^2} \quad \text{under} \quad \PROB{e^{-x}R}{ \cdot \vert N_R>0 } \xrightarrow[R \to \infty]{\mathrm{(d)}} \mathbf{N} \quad \text{under} \quad \P_{x}.
\]
Let's see where we go from here. Specifically, what limiting law can we obtain?

Let us denote by $m_x = \EXPECT{x}{\mathbf{N}}$.

We start by noticing that for all $R>0$ and $x>0$, $\EXPECT{e^{-x}R}{N_R} = 1$ (usual trick that translates the expectation to an expectation w.r.t. a single Brownian trajectory). From the convergence of $\EXPECT{e^{-x}R}{N_R /R^2 \vert N_R>0}$, we deduce that
\[
R^2 \PROB{e^{-x}R}{ N_R>0 } \to \frac{1}{m_x}.
\]

Let $t<0$ and $x,y >0$. We will denote by $\varphi_x(t) = \EXPECT{x}{e^{t \mathbf{N}}}$. We have
\begin{align*}
& \EXPECT{e^{-x-y}R}{\exp \left( \frac{t}{R^2} N_R \right) }
= \EXPECT{e^{-x-y}R}{ \EXPECT{e^{-x}R}{ \exp \left( \frac{t}{R^2} N_R \right) }^{N_{e^{-x}R}} } \\
& = \EXPECT{e^{-x-y}R}{ \left( 1 + \PROB{e^{-x}R}{N_R >0} \EXPECT{e^{-x}R}{ \exp \left( \frac{t}{R^2} N_R \right) - 1 \Big\vert N_R>0 } \right)^{N_{e^{-x}R}} } \\
& = \EXPECT{e^{-x-y}R}{ \left( 1 + \frac{1+o(1)}{R^2 m_x} (\varphi_x(t) - 1) \right)^{N_{e^{-x}R}} } \\
& = \EXPECT{e^{-x-y}R}{ \exp \left( (1+o(1)) \frac{N_{e^{-x}R}}{(e^{-x}R)^2} \frac{1}{e^{2x} m_x} (\varphi_x(t) - 1) \right) } \\
& = 1 + \frac{1+o(1)}{(e^{-x}R)^2 m_y} \left\{ \varphi_y \left( \frac{1+o(1)}{e^{2x} m_x} (\varphi_x(t) - 1) \right) - 1 \right\}
\end{align*}
But we also have
\[
\EXPECT{e^{-x-y}R}{\exp \left( \frac{t}{R^2} N_R \right) }
= 1 + \frac{1+o(1)}{R^2 m_{x+y}} (\varphi_{x+y}(t) - 1),
\]
so we have shown that
\[
\frac{1}{m_{x+y}} (\varphi_{x+y}(t)-1) = \frac{e^{2x}}{m_y} \left\{ \varphi_y \left( \frac{1}{e^{2x} m_x} (\varphi_x(t) - 1) \right) - 1 \right\}.
\]
Defining
\[
u_{x}(t) := \frac{1}{m_x e^{2x}} ( \varphi_x(t) - 1)
= \frac{1}{m_x e^{2x}} \EXPECT{x}{e^{t \mathbf{N}} - 1},
\]
this can be rewritten as
\[
u_{x+y} = u_y \circ u_x.
\]

Note that $u_x(t) \sim e^{-2x} t$ as $t \to 0$. I don't like this $e^{-2x}$. Indeed, if the above equation held for $\frac{1}{m_x} (\varphi_x - 1)$, then I would be able to show that
\[
\frac{1}{m_x} (\varphi_x(t) - 1) = \frac{t}{1-m_x t}, \quad t <0
\]
and furthermore that $m_x = m_1 x$. See Lemma \ref{L:u_circ_u} below. This would imply that $\EXPECT{x}{e^{t \mathbf{N}}} = 1/(1-m_1 x t)$, i.e. that $\mathbf{N}$ under $\P_x$ is an exponential random variable with  mean $m_1 x$.

\begin{lemma}\label{L:u_circ_u}
For all $x>0$, let $u_x : (-\infty,0) \to (-\infty,0)$ be a map analytic in some neighbourhood of the origin. Assume that for all $x,y>0$, $u_{x+y} = u_x \circ u_y$. Assume further that for all $x>0$, $u_x(t) \sim t$ as $t \to 0$, $|u_x''(0)|$ is bounded in a neighbourhood of the origin and that for all $n \geq 3$, $|u_x^{(n)}(0)| / x \to 0$ as $x \to 0$. 
Then there exists $m>0$ such that for all $x>0$ and $t<0$,
\[
u_x(t) = \frac{t}{1-mxt}.
\]
\end{lemma}

In our setting, it is natural to expect that $\EXPECT{x}{\mathbf{N}^{n-1}} \leq \tilde{C}_n x^{n-1}$ for $x$ small enough. This would directly imply that $|u_x^{(n)}(0)| \leq C_n x^{n-1}$ for $n \geq 2$, which is stronger than what is assumed in the lemma.

\begin{proof}
We expand $u_x$ around the origin:
\[
u_x(t) = t + \sum_{n \geq 2} c_n(x) t^n.
\]
The equation $u_{x+y} = u_x \circ u_y$ implies that $c_2(x+y) = c_2(x) + c_2(y)$. Since we know that $c_2$ is bounded near the origin, it implies that $c_2$ is linear: there exists $m>0$ such that $c_2(x) = mx$ for all $x >0$.
We then look at the third coefficient and obtain the equation
\[
c_3(x+y) = c_3(x) + c_3(y) + 2m^2 xy, \quad x,y>0.
\]
This implies that the map $c_3(x) - m^2 x^2$ is additive. By assumption this map is of smaller order than $x$ as $x \to 0$, so it is identically equal to 0, i.e. $c_3(x) = m^2 x^2$. In general, we can proceed by induction to show that for all $n \geq 2$, $c_n(x) = m^{n-1} x^{n-1}$. We obtained that for $t$ small enough,
\[
u_x(t) = t \sum_{n=0}^\infty (mxt)^n = \frac{t}{1-mxt}
\]
as desired.
\end{proof}

\subsection{Combining the two previous sections}

If
\[
R^2 \left\{ 1 - \EXPECT{e^{-x}R}{ \left(1-\frac{t_0}{R^2} \right)^{N_R} } \right\}
\]
indeed does not depend on $R$ and if $N_R/R^2$ under $\P_{e^{-x}R}(\cdot \vert N_R>0)$ converges to an exponential random variable, we should be able to in particular say that
\[
\EXPECT{e^{-x}R}{ \exp \left( \frac{t_0}{R^2} N_R \right) \Big\vert N_R >0 }
\]
is very close to the Laplace transform of an exponential r.v. We could then use the Tauberian theorem to obtain tail estimates.

==> sections_tex_files/old_stuff.tex <==

***********

Let $R>0$ be large, $x>0$ and $r = R/e^{x}$. Recall that we start a critical BBM with a single particle on the sphere $\partial B(0,r)$ and we kill the particles which hit $\partial B(0,R)$. We are interested in the tail of the number $N$ of pioneers on the unit sphere. Let
\begin{equation}
m_{r,R} = \frac{1}{2} \left( \log r - \log \left( 1 - \frac{\log r}{\log R} \right) + 1 \right)
= \frac{1}{2} \left( \log r + \log \left( 1+ \frac{\log r}{x} \right) + 1 \right)
\end{equation}
We will see that $\EXPECT{r,R}{N} = m_{r,R} + o(1)$.

The following lemma encapsulate the main estimate needed to obtain Theorem \ref{T:maintail4}.


\begin{lemma}\label{L:tail_key}
For any $\eps >0$, there exists $x_0 >0$ large enough so that for all $x \geq x_0$, for all $R$ large enough (depending on $x$), letting $r = e^{-x} R$, we have
\begin{equation}
\label{E:L_tail}
\PROB{r,R}{N \geq \frac{1}{x} m_{r,R} \log r} \geq r^{- (1+\eps) /x}.
\end{equation}
\end{lemma}

\begin{proof}[Proof of Lemma \ref{L:tail_key}]
Let $\eps >0$ and let $\delta >0$ be as in Tom's theorem for $c=3.5$ and $C=4.5$. By Lemmas \ref{L:g_small_lambda} and \ref{L:C_lambda}, for all $\mu \in [1,2]$,
\[
\lim_{x \to \infty} x g_{\lambda=\mu/x}(x) \to \frac{-2}{1+4/\mu}
\quad \text{and} \quad \lim_{x \to \infty} \frac1x C_{\lambda = \mu/x} = \frac{4}{\mu}
\]
uniformly in $\mu \in [1,2]$ \red{(Uniformity)}.
We can therefore fix some $x$ large enough such that for all $\mu \in [1,2]$,
\begin{equation}\label{E:proof_tail1}
\frac{e^{-\delta}}{x+ \log x + C_{\lambda = \mu/x}} \leq \frac{1}{2} \abs{ g_{\lambda = \mu/x}(x) } \leq \frac{e^\delta}{x+ \log x + C_{\lambda = \mu/x}}
\end{equation}
and such that \red{(continuity of $C_\lambda$)}
\begin{equation}
\label{E:proof_tail2}
\left\{ 1 + \frac{\log x}{x} + \frac{1}{x} C_{\lambda = \mu/x} \right\}_{\mu \in [1,2]} \supset [3.5,4.5]
\end{equation}
%\[
%\frac{2 e^{-\delta}}{1+4/\mu} \frac{1}{x} \leq \abs{g_{\lambda=\mu/x}(x)} \leq \frac{2 e^\delta}{1+4/\mu} \frac{1}{x}
%\quad \text{and} \quad
%e^{-\delta} \frac{4}{\mu} x \leq C_{\lambda = \mu/x} \leq e^\delta \frac{4}{\mu} x.
%\]
Recall that for all $\lambda \in [1/x,2/x]$,
\[
1 - \EXPECT{r,R}{ \left( 1 - g_\lambda(L) \right)^N }
= \frac{1}{r^2} g_\lambda(x).
\]
Since $\PROB{r,R}{N>0} \sim \frac{2}{r^2 \log r} $, this gives
\[
\EXPECT{r,R}{ \left( 1 - g_\lambda(L) \right)^N \big\vert N>0 } \sim \frac{L}{2} |g(x)|.
\]
By Theorem \ref{T:gh}, 
\[
g_\lambda(L) = \frac{-2}{L + \log L + C_\lambda +o(1)},
\]
where, here and in what follows, $o(1) \to 0$ as $L \to \infty$, uniformly in $\lambda \in [1/x,2/x]$
\red{(Uniformity in a compact interval)}.
Hence, one can check using the definition of $m_{r,R}$ that
\[
\left( 1 - g_\lambda(L) \right)^{m_{r,R}} = \exp \left( 1 - \frac{x + \log x + C_\lambda +o(1)}{L} \right).
\]
Wrapping things up and using \eqref{E:proof_tail1}, we have for all $\lambda \in [1/x,2/x]$,
\begin{align*}
\EXPECT{r,R}{
\exp \left\{ \left( 1 - \frac{x + \log x + C_\lambda +o(1)}{L} \right) \frac{N}{m_{r,R}} \right\} }
\sim \frac{L}{2} |g(x)|
= e^{\pm \delta} \frac{L}{x + \log x + C_\lambda}.
\end{align*}
We now rephrase the above estimate to see how we use it in Tom's theorem context. Recall \eqref{E:proof_tail2}.
Let $T = L/x$, $X= N/m_{r,R}$, $c=3.5, C=4.5$. If $L$ is large enough, we have for all $u \in [c,C]$,
\[
\frac{e^{-\delta} T}{u} \leq \Expect{ e^{(1-\frac{u}{T})X} } \leq \frac{e^\delta T}{u}.
\]
This is exactly the assumption of Theorem *** which gives that
\[
\PROB{n,R}{ \frac{N}{m_{r,R}} \geq (1-\eps) \frac{L}{x} } \geq \frac{\eps L}{2x} e^{-(1+\eps) L/x }.
\]
\end{proof}


\begin{proof}[Proof of Theorem \ref{T:maintail4}]
Let $\eps >0$. Let $x_0 >0$, $R>0$ and denote by $r_0 = R/e^{x_0}$. Assume that $x_0$ and $R$ are large enough (both depending on $\eps$) such that
\begin{equation}
\label{E:proof_T_tail}
\PROB{r_0,R}{N \geq \frac{1}{x_0} (\log R)^2 } \geq R^{-(1+\eps)/x_0}.
\end{equation}
This is a slight rephrasing of \eqref{E:L_tail}.
Let $a>0$, $x >0$ and denote by $r = R/e^x$.
Starting from a single particle on the sphere of radius $r$, we can first condition on the event that the branching process emanating from this particle contains at least $\ceil{ax_0}$ individuals which hit the sphere of radius $r_0$. This occurs with some positive probability which is uniformly bounded away from zero as $R \to \infty$ ($a$ and $x_0$ are fixed). Conditionally on this event, to create at least $a(\log R)^2$ pioneers on the unit sphere, we can ask each of the $\ceil{ax_0}$ particles to create at least $\frac{1}{x_0} (\log R)^2$ pioneers. By \eqref{E:proof_T_tail} this probability is at least
\[
(R^{-(1+\eps)/x_0})^{\ceil{ax_0}} \geq R^{-(1+\eps) (a +1/x_0)}.
\]
Because $\eps$ and $x_0$ can be chosen arbitrarily small and large respectively, this concludes the proof.
\end{proof}


\begin{comment}
******************Below is rubbish***************


Let $\lambda \in [1,2]$ and let $g_\lambda$ be the solution to
\[
\left\{
\begin{array}{l}
g_\lambda'' + 2g_\lambda' = g_\lambda^2 \\
g_\lambda(0) = 0 \\
g_\lambda'(0) = - \lambda
\end{array}
\right.
\]
By Theorem \ref{T:g}, there exists $C_\lambda \in \R$ such that
\[
\frac12 g_\lambda(x) = \frac{-1}{x} + \frac{\log x + C_\lambda}{x^2} + o(x^{-2})
= \frac{-1}{x + \log x + C_\lambda} + o(x^{-2})
\quad \quad \text{as~} x \to \infty.
\]
Claim: $\lambda \in [1,2] \mapsto C_\lambda$ is strictly decreasing and continuous.

Let $\eps >0$. We are going to apply \red{(Proposition ***)} with $c = -C_{\lambda=2}$ and $C=- C_{\lambda=1}$. Let $\delta>0$ from that proposition. Let $x_0$ be such that for all $x > x_0$, for all $\lambda \in [1,2]$, \red{(why can I choose $x_0$ uniformly in $\lambda$?)}
\begin{equation}
\label{E:proof_consequence1}
\abs{ \log |g_\lambda(x_*)| - \log |g_{\lambda=1}(x_*)| }
\leq \delta.
\end{equation}
This is possible because as $x_* \to \infty$,
\[
\log \frac{g_\lambda(x_*)}{g_{\lambda=1}(x_*)} = \log \frac{x_* + \log x_* + C_{\lambda=1} +o(1)}{x_* + \log x_* + C_{\lambda} + o(1)} = (1+o(1)) \frac{|C_{\lambda=1} - C_{\lambda}|}{x_* + \log x_*}.
\]
Let $x_* > x_0$ and $r = R/e^{x_*}$ as before. Below we denote by $L=\log R$.
For all $\lambda \in [1,2]$, we have
\[
1 - \EXPECT{r,R}{ \left( 1 - g_\lambda(L) \right)^N }
= \frac{1}{r^2} g_\lambda(x_*).
\]
Since $\PROB{r,R}{N>0} \sim \frac{2}{r^2 \log r} $, this gives
\[
\EXPECT{r,R}{ 1 - \left( 1 - g_\lambda(L) \right)^N \big\vert N>0 } \sim \frac{L}{2} g(x_*)
\]
Now, \red{here take $m = \frac{1}{2} (L + \log L)$}
\[
\left( 1 - g_\lambda(L) \right)^{m_{r,R}} = \exp \left( 1 - \frac{C_\lambda + 1 +o(1)}{L} \right)
\]
where $o(1) \to 0$ as $R \to \infty$. Hence
\begin{equation}
\EXPECT{r,R}{ 1 - \exp \left( \left( 1 - \frac{C_\lambda +1 +o(1)}{L} \right) \frac{N}{m_{r,R}} \right) \big\vert N>0 } \sim \frac{L}{2} g_\lambda(x_*).
\end{equation}
By \eqref{E:proof_consequence1}, this implies that for all $\lambda \in [1,2]$, when $R$ is large enough,
\[
e^{-\delta} \frac{L}{2} |g_{\lambda=1}(x_*)| \leq
\EXPECT{r,R}{ \exp \left( \left( 1 - \frac{C_\lambda +1}{L} \right) \frac{N}{m_{r,R}} \right) \big\vert N>0 } \leq e^{\delta} \frac{L}{2} |g_{\lambda=1}(x_*)|
\]
The right hand side is not $L/(C_\lambda+1)$... It still has to depend a bit on the constant we put in the expectation.

***********

and if $R$ is large enough,
\[
\frac{-e^{-\delta} }{x_* + \log x_* + C_\lambda} \leq
\EXPECT{r,R}{ 1 - \exp \left( \left( 1 - \frac{x_* + \log x_* + C_\lambda}{L} \right) \frac{N}{m_{r,R}} \right) \big\vert N>0 }
\leq \frac{-e^{\delta} }{x_* + \log x_* + C_\lambda}
\]
We have verified the hypothesis of Proposition ***. Therefore,
\[
\PROB{r,R}{ \frac{N}{m_{r,R}} \geq (1-\eps) L } \geq \frac{\eps L}{2} e^{-(1+\eps)L }
\]
\red{
Not really: the problem is that the constant $x_* + \log x_* + C_\lambda$ depends on $x_*$, so we are effectively looking at very high constants which is not the framework of Tom's result.}
*************End of rubbish stuff**************
\end{comment}


==> sections_tex_files/tauberian_attempt_one_point.tex <==
The following is a variation on the result Tom sent in his separate document, in which we have weakened the assumption. 

\begin{proposition}
For all $0< \eps<1$, for all $c, C>0$, there exists $\delta>0$ such that: for all $T>1$, for all random variables $X$ such that \textbf{there exists} $\lambda \in [1 - C/T, 1- c/T]$ with 
$$
\frac{e^{-\delta}}{1 - s} \le \E[ e^{s X} ] \le \frac{e^{\delta}}{1-s},
$$
then we have 
\begin{equation}\label{Eq:Taub}
\P ( X \in [(1- \eps)T, (1+ \eps) T ] ) \ge q \eps T \exp ( - (1+ \eps) T),
\end{equation}
where $q$ depends only on $c$ and $C$. 
\end{proposition}

The surprise is that it suffices to control the Laplace transform at a single point to get the result. (Tom's version assumed control of the Laplace transform over the entire interval $[1- C/T, 1- c/T]$.) This is a little surprising (but correct, I hope!, and not entirely unreasonable after all). 


\begin{proof}
We argue by contradiction. Suppose this was not the case. Then there would exists $0<\eps<1$, constants $c, C>0$ such that for all $n\ge 1$, there is $T_n \ge 1$ and a random variable $X_n$ such that \textbf{for all} $s \in I_n: = [ 1- C/T_n, 1- c/T_n]$,
\begin{equation}\label{Eq:controlLap}
\frac{e^{-1/n}}{1 - s} \le \E[ e^{s X_n} ] \le \frac{e^{1/n}}{1-s},
\end{equation}
yet 
\begin{equation}\label{Eq:Taub_contra}
\P ( X_n \in [(1- \eps)T_n, (1+ \eps) T_n ] ) \le q \eps T_n \exp ( - (1+ \eps) T_n),
\end{equation}
where $q = q(c,C)$ will be defined in the proof. Call $\phi_n(s) = \E( e^{s X_n})$ the Laplace transform of $X_n$. Set $s_n = 1- ( c+ C)/(2T_n)$ and note that $ 1- s_n = O ( 1/T_n)$. Let $Z_n$ denote a random variable whose law is that of $(1-s_n) X_n$ under 
$$d\Q = \frac{e^{s_n X_n}}{\E( e^{s_n X_n})} d\P.
$$ 
That is, for any Borel set,
$$
\Q ( Z_n \in A) = \E_\P \left[ 1_{ \{(1-s_n )X_n \in A\}}  \frac{e^{s_n X_n}}{\E( e^{s_n X_n})} \right].
$$
Fix a small constant $c_1$ and note that if $|\lambda| \le c_1$, and note that 
\begin{align*}
\E_\Q ( e^{\lambda Z_n} ) &= \frac{\E_\P [ e^{s_n X_n} e^{\lambda (1-s_n) X_n} ]}{\E_\P [e^{s_n X_n} ]}\\
& = \frac{\phi_n ( s_n + \lambda (1- s_n)) }{\phi_n ( s_n)}
\end{align*}
If $|c_1|$ is chosen small enough (depending solely on $c$ and $C$), then for all $\lambda \in [-c_1, c_1]$, the number $s = s_n + \lambda (1- s_n)$ belongs to the interval $ I_n =  [ 1- C/T_n, 1- c/T_n]$ in which we control $\phi_n$. Hence, applying the assumption \eqref{Eq:controlLap} to $\phi_n$ both at $s = s_n + \lambda (1- s_n)$ and $s = s_n$ gives us 
\begin{align*}
\E_\Q ( e^{\lambda Z_n} ) &= \frac{e^{O(2/n)}}{1 - (s_n + \lambda(1-s_n))} (1- s_n) \\
& = [1+ O(1/n)] \frac1{1- \lambda},
\end{align*}
for all $\lambda \in [ - c_1, c_1]$. Since this is a nonempty interval, which contains zero, and since the limit is the Laplace transform of an exponential random variable $Z$ with mean 1, we deduce that $Z_n$ converges to $Z$ in distribution. Therefore, if $a>0$, we deduce that 
\begin{equation}\label{Eq:controlZ}
\liminf_{n \to \infty} \Q( Z_n \in [a(1 - 2 \eps), a(1+ 2\eps)] ) \ge \Q ( Z \in [a(1- \eps), a(1+ \eps)]) \ge 2\eps e^{ - a ( 1+ \eps)}  .
\end{equation}
Now observe that 
\begin{align*}
\P ( \tfrac{X_n}{T_n} \in [1 -2 \eps, 1+2\eps] ) & \ge \E \left[ 1_{\{\tfrac{X_n}{T_n} \in [1- 2\eps, 1+2\eps]\}} \frac{e^{s_n X_n}}{ \E(e^{s_n X_n})} \right] \times e^{ - s_n T_n(1+ \eps)} \phi_n (s_n)\\
& = \Q \left[ \tfrac{Z_n}{(1-s_n) T_n} \in [1- 2\eps, 1+ 2\eps] \right]  \times e^{ - s_n T_n (1+ \eps)} \phi_n (s_n)
\end{align*}
Now, $(1- s_n) T_n = a := (c+ C)/2$, so that for $n$ large enough, 
\begin{align*}
\P ( \tfrac{X_n}{T_n} \in [1 -2 \eps, 1+2\eps] ) &\ge \Q (Z_n /a 
\in [1-2\eps, 1+2\eps] )  \times e^{ - s_n T_n  (1+ 2\eps)} \phi_n (s_n)\\
& \ge 2 \eps e^{ - a (1+ \eps)}  e^{ - T_n ( 1+ \eps) } e^{- 1/n} \frac{2 T_n}{c+ C} 
\end{align*}
This is a contradiction with \eqref{Eq:Taub_contra} if we choose $ q = 2e^{-2a}  / ( c+ C)$ (which, as required, depends only on $c$ and $C$ since $a = (c+ C)/2$).  
\end{proof}


